A Partially Ordered Structure and a Generalization of the Canonical Partition for General Graphs with Perfect Matchings

This paper is concerned with structures of general graphs with perfect matchings. We first reveal a partially ordered structure among factor-components of general graphs with perfect matchings. Our second result is a generalization of Kotzig's canonical partition to a decomposition of general graphs with perfect matchings. It contains a short proof for the theorem of the canonical partition. These results give decompositions which are canonical, that is, unique to given graphs. We also show that there are correlations between these two and that these can be computed in polynomial time.

==> isaac2012_proof_of_add.tex <==
\begin{proof}%[Theorem~\ref{thm:add}]
%Suppose $G_1\not\yield G_2$ in $G$.
First we prove  the case where there is an edge $xy$ such that $x\in V(G_1)$ and $y\in V(G_2)$.
Let $M$ be a perfect matching of $G$.
Choose a vertex $w\in V(G_2)$ such that  $w\not\gsim y$ in $G_2$,
and let $P$ be an $M$-saturated path between $w$ and $y$.
If $xw\in E(G)$,
there is an $M$-ear $xy + P + wx$ relative to $G_1$ and through $G_2$,
which means $G_1\yield G_2$ by Theorem~\ref{thm:equivalentdefinition}.
%a contradiction by Theorem~\ref{thm:equivalentdefinition}. 
% 
Thus $xw\not\in E(G)$.
%If $\mathcal{G}(G+xw) = \mathcal{G}(G)$, the claim follows.
%
Suppose $\mathcal{G}(G+xw) \neq \mathcal{G}(G)$.
%Otherwise, that is, if $\mathcal{G}(G+xw) \neq \mathcal{G}(G)$,
% there is an $M$-alternating circuit $C$ containing $xw$ in $G + xw$.
%Theorefore it suffice to consider the case where $\mathcal{G}(G+xw) \neq \mathcal{G}(G)$. 
Then there is an $M$-alternating circuit $C$ containing $xw$ in $G + xw$.
Give an orientation to $C$ so that it becomes a dicircuit with the arc $xx'$.
Trace $C$ from $x$  
and let $z$ be the first vertex we encounter that is in $V(G_2)$. 
Then $xy + xCz$ is an $M$-ear of $G$ which is relative to $G_2$
and through $G_1$, which means $G_2\yield G_1$ by Theorem~\ref{thm:equivalentdefinition},
 a contradiction to the minimality of $G_1$. 
Thus $\mathcal{G}(G+xw) = \mathcal{G}(G)$ and  we are done for this case.

Now we prove the other case,
where there is no edge of $G$ connecting $G_1$ and $G_2$.
Choose any $x\in V(G_1)$ and $y\in V(G_2)$.
If $\mathcal{G}(G + xy ) = \mathcal{G}(G)$, 
we can reduce it to the first case and the claim follows.
%
%Suppose $\mathcal{G}(G + xy ) \neq \mathcal{G}(G)$.
Therefore it suffices to consider the case that $\mathcal{G}(G + xy ) \neq \mathcal{G}(G)$. 
%If $\mathcal{G}(G + xy ) \neq \mathcal{G}(G)$,
Then, for any perfect matching $M$ of $G$,
there is an $M$-alternating circuit $C$  in $G+xy$ containing $xy$.
Give an orientation to $C$ so that it becomes a dicircuit with the arc $yy'$.
Trace $C$ from $y$ 
and let $u$ be the first vertex of $G_1$, 
and let $v$ be the first vertex in $G_2$ 
if we trace $C$ from $u$ in the opposite  direction.
%

If $\mathcal{G}(G + uv) = \mathcal{G}(G)$, the claim follows by the same argument.
%
Otherwise, that is, if  $\mathcal{G}(G + uv) \neq \mathcal{G}(G)$,
there is an $M$-alternating circuit  $D$ containing $uv$.
%
Give an orientation to $D$ so that it becomes a dicircuit with the  arc $uu'$.
If $uDv$ is disjoint from the internal vertices of $vCu$, 
then $uDv + vCu$ forms an $M$-alternating circuit containing 
non-allowed edges, a contradiction. 
Otherwise, 
trace $D$ from $u$  
and  let $w$ be the first vertex on $vCu - u$.

If $wCu$ has an even number of edges, 
$wCu + uDw$ is an $M$-alternating circuit of $G$, 
a contradiction.
Therefore, we assume $wCu$ has an odd number of edges.  
Let  $H\in\mathcal{G}(G)$ be such that  $w\in V(H)$.
%
Then $wCu + uDw - H$ leaves 
an $M$-ear in $G$  which is relative to $H$ and through $G_1$, 
% a contradiction to
contradicting  
the minimality of $G_1$. Thus this completes the proof. %Thus we are done for the second case.
\qed
\end{proof}

==> isaac2012_proof_of_base.tex <==
\begin{proof}%[Theorem~\ref{thm:base}]
First note that $G[\upstar{H}]/H$ is connected by Theorem~\ref{thm:equivalentdefinition},
and that it is factor-critical by Lemma~\ref{lem:ideal}.
Let $h$ be the contracted vertex of $G[\upstar{H}]/H$.
Note also that $K$ is a connected component of $G[\up{H}]$ if and only if 
there is a block (or possibly a union of blocks) $\what{K}$ of $G[\upstar{H}]/H$
such that  $K = \what{K} -h$. 
By Proposition~\ref{prop:fc_block}, $\what{K}$ is factor-critical.
%

Let $M$ be a perfect matching of $G$.
%There is an $M$-ear $P$ relative to $H$ 
%whose inner vertices are contained in $K$,
%because of Proposition~\ref{prop:fc_choise}.
We can take an $M$-ear $P$ relative to $h$ in $\what{K}$
by Proposition~\ref{prop:fc_choice}.
Let $u, v \in V(H)$ be the end vertices of $P$ in $G$.
Then there exists $S\in \pargpart{G}{H}$ such that $u, v\in S$
by Lemma~\ref{lem:ear-base}.
%
If $\Gamma(K)\cap V(H) = \{u, v\}$, we are done. %due to Lemma~\ref{lem:ear-base}.
Hence consider the case that 
%Hence it suffices to consider the case that
there exists  $w\in \Gamma(K)\cap V(H) \setminus \{u, v\}$
such that  $wz\in E(G)$ for some $z\in V(K)$.
%Suppose not, and let $w\in \Gamma(K)\cap V(H) \setminus \{u, v\}$
%such that  $wz\in E(G)$ for some $z\in V(K)$.
%
There is an $M$-balanced path $Q$ from $z$ to $h$ 
in $\what{K}$ by Proposition~\ref{prop:path2root}.
Trace $Q$ from $z$ and let $x$ be the first vertex we encounter that is on $P$.
Then  either $wz + zQx + xPu$ or $wz + zQx + xPv$ forms an $M$-ear relative to $H$ in $G$.
Thus $w\in S$ \if0 $w\gsim u$ \fi holds by Lemma~\ref{lem:ear-base}.
Therefore the claim holds.
\qed
\end{proof} 


==> isaac2012_sec_cor_base2add.tex <==
%isaac2012_sec_cor_base2add.tex
By Theorem~\ref{thm:base},
we can see that upper bounds of an induced elementary component 
are each ``attached'' to an equivalence class of the generalized canonical partition.
%
\begin{remark}
%If $G$ is a bipartite factorizable graph,
%no elementary components $G_1\yield G_2$ satisfies $G_1\yield G_2$.
%Thus Theorem~\ref{thm:order} is not a generalization of 
%the DM-decomposition, even though they have similar natures.
There are factorizable graphs where 
$\yield$ does not hold for any two induced elementary components,
in other words, where all the induced elementary components are minimal in the poset.
For example, we can see by Theorem~\ref{thm:equivalentdefinition} and 
Theorem~\ref{thm:base} that bipartite factorizable graphs are such,
which means Theorem~\ref{thm:order} is not a generalization of 
the DM-decomposition, even though they have similar natures.
\end{remark}
%
\input{partially_thm_2fc}

The following theorem shows that 
most of the factorizable graphs with $|\mathcal{G}(G)| \ge 2$, in a sense,
have non-trivial structures as posets.
%
\begin{theorem}\label{thm:add}
Let $G$ be a factorizable graph,
$G_1, G_2 \in \mathcal{G}(G)$ be
 induced elementary components for which  $G_1\yield G_2$ does not hold,
  and % and $G_1, G_2$ are minimal element of 
let $G_1$ be minimal in the poset $(\mathcal{G}(G), \yield)$.
%$G_1\in\mathcal{G}(G)$ be  minimal in the poset $(\mathcal{G}(G), \yield)$,
%and $G_2\in\mathcal{G}(G)$  such that $G_1\yield G_2$ does not hold$.
Then there are possibly identical complement edges $e, f$ of $G$  between
$G_1$ and $G_2$
such that
$\mathcal{G}(G + e + f)  = \mathcal{G}(G)$ and 
$G_1\yield G_2$ in $(\mathcal{G}(G+e+f), \yield)$.
\end{theorem}


==> isaac2012_sec_cor_op2base.tex <==
%isaac2012_sec_cor_op2base.tex
%
In this section we further analyze properties of factorizable graphs.
%which lead to the results in the later sections. 
We denote all the upper bounds of $H\in\mathcal{G}(G)$ 
in $(\mathcal{G}(G), \yield)$ as 
$\parupstar{G}{H}$ and define $\parup{G}{H}$ as $\parupstar{G}{H}\setminus \{H\}$.
We sometimes omit the subscripts 
if they are  apparent from the context.
For simplicity, we sometimes denote the subgraph induced by the vertices in $\up{H}$
 (resp. $\upstar{H}$) as just  
$G[\up{H}]$ (resp. $G[\upstar{H}]$), 
and the vertices of $\up{H}$ (resp. $\upstar{H}$) 
as just $V(\up{H})$ (resp. $V(\upstar{H})$).
%
\begin{lemma}\label{lem:ear-base}
Let $G$ be a factorizable graph, $M$ be a perfect matching of $G$,
and $H\in \mathcal{G}(G)$.
Let $P$ be an $M$-ear relative to $H$ with end vertices 
$u, v \in V(H)$.
Then $u\gsim v$.
\end{lemma}
\begin{proof}
Suppose the claim fails, that is, $u\neq v$ and 
there is an $M$-saturated path $Q$ between $u$ and $v$.
Trace $Q$ from $u$ and let $x$ be the first vertex we encounter that is  on $P-u$.
If $uPx$ has an even number of  edges,
$uQx + xPu$ is an $M$-alternating circuit containing non-allowed edges,  a contradiction.
Hence we  suppose  $uPx$ has an odd number of  edges.
Let $I\in \mathcal{G}(G)$ be such that  $x\in V(I)$.
Then one of the components of $uQx + xPu - E(I)$ is  an $M$-ear relative to $I$ and through $H$,
a contradiction by Theorem~\ref{thm:equivalentdefinition}.
\qed
\end{proof}  
%
%
\begin{proposition}\label{prop:union}
Let $G$ be a graph and $M$ be a matching of $G$. 
Let $H_1, H_2\subseteq G$ be factor-critical subgraphs of $G$ such that 
there exists $v\in V(H_1)\cap V(H_2)$ and that 
for each $i = 1, 2$, 
$M_{H_i}$ is a near-perfect matching of $H_i$ exposing only $v$. 
Then, $H_1\cup H_2$ is factor-critical. 
\end{proposition}
\begin{proof}
Apparently, $M_1\cup M_2$ is a near-perfect matching of $H_1\cup H_2$, 
exposing only $v$. 
Since $H_1$ and $H_2$ are both factor-critical, 
the claim follows by Proposition~\ref{prop:path2root}. 
\qed
\end{proof}
%
\begin{lemma}\label{lem:ideal}
Let $G$ be a factorizable graph, and $H\in\mathcal{G}(G)$. 
Then, $G[\upstar{H}]/H$ is factor-critical. 
\end{lemma}
\begin{proof}
Let $M$ be a perfect matching of $G$. 
Let $\mathcal{X}\subseteq 2^{V(G)}$ be the family of 
separable set for $H$. 
Then, by Theorem~\ref{thm:order}, 
$\bigcup_{X\in\mathcal{X}} X = V(\upstar{H})$. 
On the other hand, $G[\bigcup_{X\in\mathcal{X}} X ]/H$ is factor-critical 
by Proposition~\ref{prop:union}. 
Therefore,  the claim follows. 
\qed
\end{proof}
%
\begin{theorem}\label{thm:base}
Let $H$ be an induced elementary component of a \matchablesp graph $G$.
Then for each connected component $K$ of $G[\up{H}]$,
there exists $S\in \pargpart{G}{H}$ such that 
$\Gamma(K)\cap V(H)\subseteq S$.  
\end{theorem}


==> isaac2012_sec_p_2end.tex <==
%isaac2012_sec_p_2end.tex
%
\begin{theorem}\label{thm:order}
$\yield$ is a partial order.
\end{theorem}
\input{partially_proof_thm_order}
\begin{comment}
\begin{proof}
The reflexivity is obvious from the definition.
The transitivity  obviously follows from Theorem~\ref{thm:equivalentdefinition}.
Hence, we will prove the antisymmetry.
Let $G_1, G_2\in \mathcal{G}(G)$ be such that $G_1\yield G_2$ and $G_2\yield G_1$.
%If $G_1 = G_2$, the claim follows.
Suppose the claim fails, that is, $G_1 \neq G_2$.
Let $X\subseteq \Vg$ be
a separable set for $G_1$ that contains $G_2$, and let 
 %a vertex set corresponding to the definition of $G_1\yield G_2$,
%that is, satisfying $V(G_1), V(G_2)\subseteq X$,
%for any $H\in\mathcal{G}(G)$ $V(H)\cap X = \emptyset$ or $V(H)\subseteq X$,
% and $G[X]/G_1$ is factor-critical.
\if0 Let \fi  $M$ be a perfect matching of $G$.
Let $g_1$ be the contracted vertex of $G[X]/G_1$, and 
take an $M$-ear $P$ relative to \if0 the contracted vertex  \fi $g_1$ in $G[X]/G_1$
by Proposition~\ref{prop:fc_choice}, 
whose corresponding end vertices  in $G$ are $p$ and $q$.
%
Since $G_2\yield G_1$, by Lemma~\ref{lem:path2base},
there is an $M$-\zero path $Q$ from $p$ to some vertex in $V(G_2)$.
Trace  $Q$ from $p$ and let $x$ be the first vertex we encounter that is
in $X\setminus V(G_1)$.
Since $G[X]/G_1$ is factor-critical, 
there is an $M$-balanced  path $R$ from $x$ to $q$
whose vertices except $q$ are contained in $X\setminus V(G_1)$.
Trace  $R$ from $x$ and let $y$ be the first vertex we encounter that is on $P$.
If $pPy$ has an even number of edges, 
$pQx + xRy + yPp$ is an $M$-alternating circuit containing non-allowed edges, 
a contradiction.

%So suppose $pPw$ has odd edges.
Hence hereafter we assume $pPw$ has an odd number of edges.
By Proposition~\ref{prop:nonpositive},
there is an $M$-saturated or balanced path $L$ from $q$ to $p$
which is contained in $G_1$.
Trace $L$ from $q$ and let $w$ be the first vertex on $Q$.
If $pQw$ has an odd number of edges, then
$wQp + P + qLw$ is an $M$-alternating circuit, a contradiction.
If  $pQw$ has an even  number of edges,
then $qLw+ wQx + xRy + yPq$ is an $M$-alternating circuit,
which is also a contradiction.
Thus we get $G_1 = G_2$, and  the claim follows.
\qed
\end{proof}
\end{comment}


==> isaac2012_sec_p_nonpositive2equivalentdefinition.tex <==
%isaac2012_sec_p_nonpositive2equivalentdefinition.tex
%
%
Let $G$ be a factorizable graph and $M$ be a perfect matching of $G$.
We call a sequence of induced elementary components
$H_0,\ldots, H_k \in \mathcal{G}(G)$  an 
\textit{$M$-ear sequence from $H_0$ to $H_k$}
if there is an $M$-ear relative to $H_{i-1}$ and through $H_i$ 
for each $i = 1,\ldots, k-1$.
%

%
%
The next theorem gives an equivalent definition of $\yield$. 
%
\if0%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
and appears in proving 
Theorem~\ref{thm:order},
however, much more important point is, as we later see, that it is  the 
key to polynomial time algorithm for computing $\yield$.
\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\begin{theorem}\label{thm:equivalentdefinition}
Let $G$ be a factorizable graph, 
$M$ be a perfect matching of $G$, and 
 $G_1, G_2\in\mathcal{G}(G)$.
Then, $G_1\yield G_2$ if and only if 
there exists %a sequence $G_1=H_0, H_1,\ldots,H_k = G_2$ which satisfies
an $M$-ear sequence from $G_1$ to $G_2$.
%\begin{quote}
%$\clubsuit$
%for each $0 \le i \le k-1$ there exists an $M$-ear $P_i$ relative to $H_i$.
%\end{quote}
\end{theorem}


==> isaac2012_sec_p_op2nonpositive.tex <==
%isaac2012_sec_p_op2nonpostivie.tex
In this section we show our first result: a partially ordered structure among 
induced elementary components of factorizable graphs.
%
For a factorizable graph $G$ \if0 , $X\subseteq V(G)$, \fi and $G_1\in\mathcal{G}(G)$,
we call $X\subseteq V(G)$ a \textit{separable set for} $G_1$
if each $H\in \mathcal{G}(G)$ satisfies $V(H)\subseteq X$ or $V(H)\cap X = \emptyset$,
and  $G[X]/G_1$ is factor-critical.
%
\begin{definition}
Let $G$ be a factorizable  graph and $G_1, G_2 \in \mathcal{G}(G)$.
We say $G_1\yield G_2$ if there exists  a separable set $X\subseteq \Vg$ for $G_1$
that contains $G_2$.
%We say $G_1\yield G_2$ if there exists $X\subseteq \Vg$ 
%such that $V(G_1), V(G_2)\subseteq X$,
%each $H\in \mathcal{G}(G)$ satisfies $V(H)\subseteq X$ or $V(H)\cap X = \emptyset$,
%and 
%$G[X]/G_1$ is factor-critical.
\end{definition}
%
%
\begin{lemma}\label{lem:path2base}
Let $G$ be a factorizable graph and 
$M$ be a perfect matching of $G$.
Let $G_1,G_2\in\mathcal{G}(G)$ such that  $G_1\yield G_2$ and 
  $X\subseteq V(G)$ be a separable set for $G_1$ that contains $G_2$.
Then for any $u\in V(G_2)$ there exists $v\in V(G_1)$ 
such that  there is an $M$-\zero path from $u$ to $v$
whose vertices except $v$ are contained in $X\setminus V(G_1)$.
\end{lemma}
\begin{proof}
Since $M_{X\setminus V(G_1)}$ 
is a near-perfect matching of $G[X]/G_1$ 
that exposes the contracted vertex $g_1$ corresponding to $G_1$,
we are done by Proposition~\ref{prop:path2root}.
\qed
\end{proof}
%
\if0%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:path2base}
Let $G$ be a factorizable graph and 
$M$ be a perfect matching of $G$.
Let $G_1,G_2\in\mathcal{G}(G)$ satisfy $G_1\yield G_2$ and 
  $X\subseteq V(G)$ be the set of vertices 
 where $V(G_1), V(G_2)\subseteq X$,
each $H\in \mathcal{G}(G)$ satisfies $V(H)\subseteq X$ or $V(H)\cap X = \emptyset$,
and 
$G[X]/G_1$ is factor-critical.
Then for any $u\in V(G_2)$ there exists $v\in V(G_1)$ 
where there is an $M$-\zero path from $u$ to $v$
whose vertices except $v$ are contained in $X\setminus V(G_1)$.
\end{lemma}
\begin{proof}
As $M_{X\setminus V(G_1)}$ 
is a near-perfect matching of $G[X]/G_1$ 
that exposes the contracted vertex $g_1$ corresponding to $G_1$,
we are done by Proposition~\ref{prop:path2root}.
\end{proof}
\fi%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{proposition}\label{prop:nonpositive}
Let $G$ be an elementary graph and $M$ be a perfect matching of $G$.  
Then for any two vertices $u,v \in V(G)$
there is an $M$-saturated path between $u$ and $v$, 
or an $M$-\zero path from $u$ to $v$.
\end{proposition}


==> isaac2012_sec_pre_note.tex <==
Later on this paper, note the following fundamental properties;
for a factorizable graph $G$ and its perfect matching $M$,
$e\in E(G)\setminus M$ is allowed if and only if 
there is an $M$-alternating circuit containing $e$;
for $u,v\in V(G)$,  $G-u-v$ is factorizable 
if and only if there is an $M$-saturated path 
between $u$ and $v$;
for two $M$-alternating path $P$ and $Q$,
a segment of $P\cap Q$ is an $M$-saturated paths if 
it  contains no end vertices of $P$ nor $Q$. 


==> partially_prop_proof_nonpositive.tex <==
%partially_prop_proof_nonpositive
\begin{proposition}\label{prop:nonpositive}
Let $G$ be an elementary graph and $M$ be a perfect matching of $G$.  
Then for any two vertices $u,v \in V(G)$
there is an $M$-saturated path between $u$ and $v$, 
or an $M$-\zero path from $u$ to $v$.
\end{proposition}
\begin{proof}
Without loss of generality we can assume $G$ is matching-covered, 
that is, every edge of $G$ is allowed.
Let $U_1\subseteq V(G)$ be the set of vertices that can be reached from $u$ by an  
$M$-saturated path,
and $U_2\subseteq V(G)$ be the set of vertices that can be reached from $u$ by an $M$-\zero path
but cannot be by any $M$-saturated paths. 
We are going to obtain the claim by showing $U:= U_1\dot{\cup} U_2 = V(G)$.
Suppose that it fails, namely that $U \subsetneq V(G)$.
Then there are $v\in U$ and $w\in V(G)\setminus U$ such that $vw\in E(G)$,
since $G$ is connected.
%As $G$ is connected, %$\Gamma(U)\neq \emptyset$.
%%Let $w\in V(G)\setminus U$ and $z\in U$ with  $wz\in E(G)$.
%there are $v\in U$ and $w\in V(G)\setminus U$ where $vw\in E(G)$.
By the definition of $U$,
there is an $M$-saturated or \zero path $P$ from $u$ to $v$, 
which satisfies $V(P)\subseteq U$ 
since for each $z \in V(P)$ 
$uPz$ is an $M$-saturated or balanced path from $u$ to $z$. 
If $P$ is $M$-saturated, therefore, 
$P+vw$ is an $M$-balanced path from $u$ to $w$, 
which means $w\in U$, a contradiction.

Hence, hereafter we  assume $P$ is $M$-balanced, from $u$ to $v$.
Since $vw$ is defined to be allowed, 
there is an $M$-saturated path $Q$ between $v$ and $w$ 
by Proposition~\ref{prop:allowed2circuit}. 
Trace $P$ from $u$ and let $x$ be the first vertex we encounter 
that is in $Q$; 
such $x$ surely exists under the current hypotheses since $v\in V(P)\cap V(Q)$. 
%
\begin{cclaim}\label{claim:u2x}
$uPx$ is an $M$-balanced path. 
\end{cclaim}
\begin{proof}
Suppose the claim fails, 
which is equivalent to $uPx$ being an $M$-saturated path. 
Then, $x'\in V(uPx)$. 
On the other hand, 
since $Q$ is $M$-saturated, $x'\in V(Q)$. 
Therefore, $x'\in V(uPx)\cap V(Q)$,  
which means we counter $x'$ before $x$ if we trace $P$ from $u$, 
a contradiction. 
\qed
\end{proof}
%
\begin{cclaim}\label{claim:x2w}
$xPw$ is an $M$-saturated path between $x$ and $w$. 
\end{cclaim}
\begin{proof}
If $x = v$, $vPx$ is a trivial $M$-balanced path from $v$ to $x$. 
Even if $x \neq v$, so is it by Proposition~$\clubsuit$. 
Anyway, whether $x = v$ or not, $vPx$ is an $M$-balanced path 
from $v$ to $x$. 
Therefore, together with $vPw$ being an $M$-saturated path, 
$xPw$ is an $M$-balanced path from $x$ to $w$. 
\qed
\end{proof}
%
By Claims~\ref{claim:u2x} and \ref{claim:x2w}, 
$uPx + xQw$ is an $M$-saturated path between $u$ and $w$, 
since $V(uPx)\cap V(xQw) = \{ x\}$ by the definition of $x$. 
Hence, $w\in U$, a contradiction, 
and we obtain $U = V(G)$, which completes the proof. 
\qed
\end{proof}

